Near-Optimal Non-Convex Stochastic Optimization under Generalized Smoothness

The generalized smooth condition, $(L_{0},L_{1})$-smoothness, has triggered people's interest since it is more realistic in many optimization problems shown by both empirical and theoretical evidence. Two recent works established the $O(\epsilon^{-3})$ sample complexity to obtain an $O(\epsilon)$-stationary point. However, both require a large batch size on the order of $\mathrm{ploy}(\epsilon^{-1})$, which is not only computationally burdensome but also unsuitable for streaming applications. Additionally, these existing convergence bounds are established only for the expected rate, which is inadequate as they do not supply a useful performance guarantee on a single run. In this work, we solve the prior two problems simultaneously by revisiting a simple variant of the STORM algorithm. Specifically, under the $(L_{0},L_{1})$-smoothness and affine-type noises, we establish the first near-optimal $O(\log(1/(\delta\epsilon))\epsilon^{-3})$ high-probability sample complexity where $\delta\in(0,1)$ is the failure probability. Besides, for the same algorithm, we also recover the optimal $O(\epsilon^{-3})$ sample complexity for the expected convergence with improved dependence on the problem-dependent parameter. More importantly, our convergence results only require a constant batch size in contrast to the previous works.

==> checklist.tex <==

\section*{Checklist}
\begin{enumerate}
\item For all models and algorithms presented, check if you include:
\begin{enumerate}
\item A clear description of the mathematical setting, assumptions, algorithm,
and/or model. {[}\textcolor{red}{Yes}/No/Not Applicable{]}
\item An analysis of the properties and complexity (time, space, sample
size) of any algorithm. {[}\textcolor{red}{Yes}/No/Not Applicable{]}
\item (Optional) Anonymized source code, with specification of all dependencies,
including external libraries. {[}Yes/\textcolor{red}{No}/Not Applicable{]}
\end{enumerate}
\item For any theoretical claim, check if you include:
\begin{enumerate}
\item Statements of the full set of assumptions of all theoretical results.
{[}\textcolor{red}{Yes}/No/Not Applicable{]}
\item Complete proofs of all theoretical results. {[}\textcolor{red}{Yes}/No/Not
Applicable{]}
\item Clear explanations of any assumptions. {[}\textcolor{red}{Yes}/No/Not
Applicable{]}
\end{enumerate}
\item For all figures and tables that present empirical results, check if
you include:
\begin{enumerate}
\item The code, data, and instructions needed to reproduce the main experimental
results (either in the supplemental material or as a URL). {[}Yes/No/\textcolor{red}{Not
Applicable}{]}
\item All the training details (e.g., data splits, hyperparameters, how
they were chosen). {[}Yes/No/\textcolor{red}{Not Applicable}{]}
\item A clear definition of the specific measure or statistics and error
bars (e.g., with respect to the random seed after running experiments
multiple times). {[}Yes/No/\textcolor{red}{Not Applicable}{]}
\item A description of the computing infrastructure used. (e.g., type of
GPUs, internal cluster, or cloud provider). {[}Yes/No/\textcolor{red}{Not
Applicable}{]}
\end{enumerate}
\item If you are using existing assets (e.g., code, data, models) or curating/releasing
new assets, check if you include:
\begin{enumerate}
\item Citations of the creator If your work uses existing assets. {[}Yes/No/\textcolor{red}{Not
Applicable}{]}
\item The license information of the assets, if applicable. {[}Yes/No/\textcolor{red}{Not
Applicable}{]}
\item New assets either in the supplemental material or as a URL, if applicable.
{[}Yes/No/\textcolor{red}{Not Applicable}{]}
\item Information about consent from data providers/curators. {[}Yes/No/\textcolor{red}{Not
Applicable}{]}
\item Discussion of sensible content if applicable, e.g., personally identifiable
information or offensive content. {[}Yes/No/\textcolor{red}{Not Applicable}{]}
\end{enumerate}
\item If you used crowdsourcing or conducted research with human subjects,
check if you include:
\begin{enumerate}
\item The full text of instructions given to participants and screenshots.
{[}Yes/No/\textcolor{red}{Not Applicable}{]}
\item Descriptions of potential participant risks, with links to Institutional
Review Board (IRB) approvals if applicable. {[}Yes/No/\textcolor{red}{Not
Applicable}{]}
\item The estimated hourly wage paid to participants and the total amount
spent on participant compensation. {[}Yes/No/\textcolor{red}{Not Applicable}{]}
\end{enumerate}
\end{enumerate}


